Sound Automation of Magic Wands (extended version)

The magic wand $\mathbin{-\!\!*}$ (also called separating implication) is a separation logic connective commonly used to specify properties of partial data structures, for instance during iterative traversals. A footprint of a magic wand formula $A \mathbin{-\!\!*} B$ is a state that, combined with any state in which $A$ holds, yields a state in which $B$ holds. The key challenge of proving a magic wand (also called packaging a wand) is to find such a footprint. Existing package algorithms either have a high annotation overhead or, as we show in this paper, are unsound. We present a formal framework that precisely characterises a wide design space of possible package algorithms applicable to a large class of separation logics. We prove in Isabelle/HOL that our formal framework is sound and complete, and use it to develop a novel package algorithm that offers competitive automation and is sound. Moreover, we present a novel, restricted definition of wands and prove in Isabelle/HOL that it is possible to soundly combine fractions of such wands, which is not the case for arbitrary wands. We have implemented our techniques for the Viper language, and demonstrate that they are effective in practice.

==> package_logic.tex <==
In this section, we present a \thibault{logical framework to build sound package algorithms.
At the core of our framework is the \emph{package logic}, which can be used as a formal basis for package algorithms:}
Packaging a wand in a given state is equivalent to finding a proof in the package logic and, thus,
a package algorithm corresponds to a proof search in the logic.
\thibault{In other words, the rules of the package logic describe the steps that a package algorithm may take to package a wand.}
%This logic is sound and complete for packaging wands, in the sense that
%a w
This logic is sound (\thmref{thm:soundness}) and complete (\thmref{thm:completeness}), in the following sense:
A computation of a footprint for a wand $A \wand B$ in the state $\sigma$ is formalised as a judgement $s$ in the logic.
The computation is valid if and only if there exists a derivation of $s$ in the logic.
%in the sense that a correct proof in the logic corresponds to a correct footprint of the wand,
%which can be extracted from the program state,
%and \emph{vice versa}.
%\footnote{As can be seen in the soundness theorem, the situation is slightly more complicated in classical SL, where one must check an additional condition on the proof to ensure that the candidate footprint is indeed a valid footprint.}

In \secref{subsec:motivation}, we show that there is no optimal strategy for a package algorithm, which is why our solution is a logic instead of a (deterministic) algorithm with a specific strategy.
% \thibault{This logic provides building blocks for designing a package algorithm.}
\tout{We then explain, in \secref{subsec:fixing}, the key ideas to fix the fundamental unsoundness of the FIB package algorithm~\cite{SchwerhoffSummers15}
(described in \secref{subsec:footprint_infer_base}) in order to get a first sound package algorithm,
which corresponds to a proof search in the package logic.}
\thibault{\secref{subsec:fixing} presents an example of a specific sound package algorithm, which is inspired by the FIB and fixes its unsoundness.
This algorithm is one instance of the algorithms described by our logic.}
% We explain in \secref{subsec:fixing} how to fix the unsoundness of the FIB described in \secref{subsec:footprint_infer_base}.
%on an example the choices a package algorithm has to make when packaging a wand,
%which motivates why we need a logic instead of a parametrised algorithm.
In \secref{subsec:prelim}, we define the state model and the assertion language used by the package logic.
The state model is \thibault{allowed to be} a separation algebra to capture different SL \thibault{flavours}.
% In particular, to support different SL and IDF extensions, the state model is simply assumed to be a separation algebra.
%, in particular this section defines the concept of a \emph{separation algebra}.
%\secref{subsec:configurations} defines the concepts used by the rules of the logic, while
\secref{subsec:logic} presents the logic.
Finally, we prove that the package logic is sound and complete in \secref{subsec:soundness-completeness}.


All results presented in this section have been mechanised in Isabelle/HOL.
In particular, the package logic we have mechanised is parametric w.r.t. the wand's semantics, \thibault{in the sense of which states are considered valid footprints}.
We propose in \secref{sec:combinable} a novel semantics for wands, which ensures that wands are combinable (an assertion $A$ is \emph{combinable} iff the entailment $A^p * A^q \models A^{p+q}$ holds).
For the sake of presentation, we use the standard definition of the wand here,
which allows us to present a simplified version of the mechanised package logic.
We show in \secref{sec:combinable} how to generalise this simplified version to handle other semantics for the wand.

%All results presented in this section (except \appref{app:extensions}) have been mechanised in Isabelle/HOL.
%We present, in this section, a simplified version of what we have mechanised in Isabelle/HOL.
%This simplification focuses on the usual definitions of wands.
%We explain in \secref{sec:combinable} how to extend this logic to handle restricted definitions of the wand.







\subsection{Using a Logic to Build Package Algorithms}\label{subsec:motivationold}

As we explained in \secref{sec:intro}, there is a wide design space for package algorithms.
%One way our solution captures this wide design space is by being parametrised in the state model, as we explain in \secref{subsec:prelim}.
One important dimension in this design space is the strategy used by an algorithm to find a footprint.
\thibault{Note that a footprint is a state, and thus a footprint corresponds to permissions to a set of heap locations \emph{and} the values contained in those heap locations.
For the sake of presentation, we often characterize a footprint only by the permissions it contains.}
There is no optimal strategy for a package algorithm, since there is in general no best footprint for a given wand, as we show below.
The strategy used by an algorithm fundamentally impacts the footprints it computes, and different strategies strike different trade-offs in the design space.

Our solution captures this dimension by being a logic instead of an algorithm with a fixed strategy, and, as such, it \thibault{embraces} many different strategies.
%Our solution captures this dimension by being a logic instead of an algorithm, and, as such, it can leverage many different strategies.
The rules of the logic correspond to the steps that a package algorithm can take to compute a footprint,
and thus these rules can be used as building blocks to build a package algorithm.
The strategy of a package algorithm corresponds to a proof search strategy in the logic.
%as we explain in \secref{subsec:logic}.
Any package algorithm constructed with these building blocks is sound, since the package logic is sound (\secref{subsec:soundness-completeness}).

\paragraph{No optimal strategy to package a wand.}
There is no optimal strategy for a package algorithm, since in general a wand $A \wand B$ holds in several different and incomparable states $\sigma_w$.
%and thus there is no best candidate for $\sigma_w$ (the footprint).
%To understand why, consider the wand $A \wand B$.
%In general, the wand $A \wand B$ holds in several different and incomparable states.
One reason is that $A \wand B$ can be satisfied by either proving directly $B$, but also by falsifying $A$.
As a simple example, \code{acc(x.f)} $\wand$ \code{acc(x.g)} holds in any state $\sigma_w$ that contains permission to either \code{x.f} or \code{x.g}.
\thibault{In a state with permission to both heap locations, a package algorithm must therefore choose which footprint to extract between these two options.}
Even if we ignore the possibility of falsifying $A$ to satisfy the wand (which would make it impossible to apply such a wand),
the wand $A \wand B$ might still not have, in general, a unique best footprint, as the next example shows.

Consider IDF with \emph{fractional permissions}~\cite{Boyland03},
i.e. where permissions are positive rationals less or equal to $1$ (and $1$ is called the \emph{full permission}),
and consider the wand $w := \code{acc(x.b, 1/2)} \wand \code{acc(x.b, 1/2)} * (\code{x.b} \Rightarrow \code{acc(x.f)})$.
To package this wand, an algorithm must choose how to satisfy the implication $\code{x.b} \Rightarrow \code{acc(x.f)}$.
One way is to choose a footprint with full permission to \code{x.f}, which is what the original FIB does.
Another way is to choose a footprint $\sigma_w^b$ \thibault{with some permission to \code{x.b} and} in which \code{x.b} contains the value false
\thibault{(recall that a footprint corresponds to permissions to a set of heap locations and the values contained in those heap locations)}.
Indeed, any state that satisfies the LHS of $w$ (\code{acc(x.b, 1/2)}) and that is compatible with $\sigma_w^b$ must also contain the value false for \code{x.b},
and thus the implication is trivially satisfied.
%In a state $\sigma$ where \code{acc(x.f) * acc(x.b, 1/2) * !b} holds,
%both $\sigma_w^f$ and $\sigma_w^b$ can be extracted from the state $\sigma$ as a footprint of the wand $w$, and
No choice of footprint, and thus no strategy, is \emph{a priori} better than the other.
Both strategies are captured by the package logic, since both strategies correspond to a proof search strategy in the logic.
%a package algorithm could thus compute  footprint either $\
%it is unclear which footprint is better








\subsection{A Sound Package Algorithm}\label{subsec:fixing}

\tout{We now explain the key ideas to solve the fundamental unsoundness of the FIB.
This gives us a concrete instance of a sound package algorithm, which corresponds to one proof search strategy in the package logic.
As explained in \secref{subsec:footprint_infer_base}, the key idea of the FIB
for a wand $A \wand B$ is to construct a state $\sigma_B$ that satisfies $B$,
where the permissions for $\sigma_B$ are guaranteed by $A$ or taken from the \emph{outer state} $\sigma$ (recall that the outer state initially corresponds to the state of the program before the package statement).
To achieve this, the FIB first constructs a state $\sigma_A$ that satisfies $A$, and then traverses $B$ to construct $\sigma_B$,
transferring permissions to satisfy $B$ from either $\sigma_A$ (preferrably) or $\sigma$ to $\sigma_B$.
The permissions taken from $\sigma$ form the footprint $\sigma_w$.
In other words, the FIB constructs a state $\sigma_w$ such that, if $\sigma_A$ and $\sigma_w$ are compatible, then $\sigma_A \oplus \sigma_w \models B$.}

\tout{However, for $\sigma_w$ to satisfy the wand $A \wand B$, the previous property must hold \emph{for all states} $\sigma_A$ that satisfy $A$.
The FIB is unsound, since it guarantees this property for \emph{one} such $\sigma_A$ only.
%
To solve this issue, instead of considering \emph{only one} state $\sigma_A$ and to construct only one corresponding state $\sigma_B$,
we consider \emph{all} states $\sigma_A$ that satisfy $A$, and construct for each a corresponding state $\sigma_B$ that satisfies $B$,
taking permissions from either $\sigma_A$ or from the outer state $\sigma$.
Thus, instead of tracking only one pair of states, $(\sigma_A, \sigma_B$), as the FIB does, we track a \emph{set} $S$ of pairs of states $(\sigma_A, \sigma_B)$.
% This way, we can ensure that the footprint we infer is indeed a valid footprint for all the states which satisfy $A$.
We call the set $S$ a \emph{witness set}, and the pair $(\sigma, S)$, composed of the outer state and a witness set, a \emph{context}.
In the rest of this paper, we use the notation $S^A$ to refer to all pairs of $S$ projected on their first element, i.e.
%to mean that we project all elements of $S$ on their first element, i.e.
$S^A := \{ \sigma_A \mid (\sigma_A, \sigma_B) \in S \}$.}

\thibault{We now describe an automatic package algorithm that corresponds to a proof search strategy in our package logic, and which is thus sound.
Consider packaging the wand $w := A \wand B$ in the state $\sigma_0$.
The goal of a package algorithm is to extract from the outer state $\sigma_0$ a footprint $\sigma_w$ such that,
for all states $\sigma_A$ that satisfy $A$, $\sigma_A \# \sigma_w \Rightarrow \sigma_A \oplus \sigma_w \models B$.
The key idea to achieve this is to explicitly consider \emph{all} states $\sigma_A$ that satisfy $A$,
and to construct, for each state $\sigma_A$, a corresponding state $\sigma_B$ that satisfies $B$, taking permissions (and values) from either $\sigma_A$ or from the outer state $\sigma_0$.
The permissions taken from $\sigma_0$ represent the footprint $\sigma_w$.
}

\thibault{To do this automatically, we consider \emph{all} states $\sigma_A$ that satisfy $A$, and construct for each a corresponding state $\sigma_B$ that satisfies $B$,
taking permissions from either $\sigma_A$ (preferrably) or from the outer state $\sigma_0$.
We achieve this by explicitly tracking a \emph{set} $S$ of pairs of states $(\sigma_A, \sigma_B)$, which we update while traversing the assertion $B$.
At any point of the algorithm, given a pair $(\sigma_A, \sigma_B) \in S$,
$\sigma_B$ represents the permissions that have been ``consumed'' to prove the initial part of $B$,
while $\sigma_A$ represents the permissions that are still ``available'' to prove the remaining part of $B$.
We call the set $S$ a \emph{witness set}, and the pair $(\sigma, S)$, composed of the outer state and a witness set, a \emph{context}.
Note that explicitly tracking this witness set is a key difference with the FIB, which tracks only one pair of states $(\sigma_A, \sigma_B)$ at a time.
In the rest of this paper, we use the notation $S^A$ to refer to all pairs of $S$ projected on their first element, i.e.
%to mean that we project all elements of $S$ on their first element, i.e.
$S^A := \{ \sigma_A \mid (\sigma_A, \sigma_B) \in S \}$.}

\tout{We now describe, on a high-level, a package algorithm that uses a witness set and follows the same strategy as the FIB.}
\thibault{More precisely,} consider packaging the wand $A \wand B_1 * \ldots B_n$ in the state $\sigma_0$.
%how an algorithm following the same strategy as the FIB can proceed to package the wand $A \wand B_1 \ldotp B_n$
Initially, the witness set $S$ contains all pairs $(\sigma_A, e)$, where $\sigma_A$ is a state that satisfies $A$ and $e$ is the empy state.
If the assertion $B$ is intuitionistic\footnote{An assertion $B$ is intuitionistic~\cite{Reynolds02a} iff, if $B$ holds in a state $\sigma$, then $B$ holds in any state $\sigma'$ larger than $\sigma$.
In intuitionistic SL or in IDF, all assertions are intuitionistic.},
then it is sufficient for $S^A$ to be a set of \emph{minimal} states $\sigma_A$ that satisfy $A$ to ensure soundness.
If $B$ is not intuitionistic, then $S^A$ must contain all states $\sigma_A$ that satisfy $A$.
%
We then traverse the assertion $B_1 * \ldots * B_n$ (RHS of the wand) from left to right, similarly to the FIB.
Assume that the current context is $(\sigma_0, S)$.
When we encounter the assertion $B_i$, we have two possible cases:
\begin{enumerate}
    \item All states $\sigma_A \in S^A$ satisfy $B_i$,
    \thibault{which means that the permissions (or values) required by $B_i$ are provided by the LHS of the wand}.
    In this case, for each pair $(\sigma_A, \sigma_B) \in S$, we transfer permissions \thibault{(and the corresponding values)} to satisfy $B_i$ from $\sigma_A$ to $\sigma_B$.
    \thibault{Note that the transferred permissions might be different for each pair $(\sigma_A, \sigma_B)$.}
    This gives us a new witness set $S'$, while the outer state $\sigma_0$ is left unchanged.
    We must then handle the next assertion $B_{i+1}$ in the context $(\sigma, S')$.
    \item There is at least one pair $(\sigma_A, \sigma_B) \in S$ such that $B_i$ does not hold in $\sigma_A$.
    \thibault{In this case, the algorithm fails if combining the permissions (and values) contained in the outer state
    with each $\sigma_A \in S^A$ is not sufficient to satisfy $B_i$.}
    \thibault{Otherwise,} we need to perform an extra step before proceeding as in the first case to prove $B_i$.
    We transfer some permissions from the outer state $\sigma_0$ to each state in $S^A$ such that $B_i$ holds in all $\sigma_A \in S^A$.
    This gives us a new context $(\sigma_0', S')$, and we can now apply the first case with the context $(\sigma_0', S')$.
\end{enumerate}
As we will explain in \secref{subsec:logic}, these two cases correspond to the application of two rules in the logic and, therefore, the algorithm corresponds to a proof search strategy.
\thibault{We show, as an example, how the above algorithm packages the wand
$\code{acc(x.f)} * (\code{x.f = y} \vee  \code{x.f = z}) \wand \code{acc(x.f)} * \code{acc(x.f.g)}$
in \appref{app:example-sound-package}.}










\subsection{Separation Algebra and Assertions}\label{subsec:prelim}

In order to capture different state models and different flavours of separation logic, the package logic is parametrised by a separation algebra.
For space reasons, we present here a simplified overview of this separation algebra, but all definitions are given in \appref{app:context} and have been mechanised in Isabelle/HOL.
We consider a separation algebra~\cite{Calcagno2007,Dockins2009} where $\Sigma$ is the set of states,
$\oplus: \Sigma \times \Sigma \rightarrow \Sigma$ is a partial operation that is commutative and associative,
and $e \in \Sigma$, which corresponds to the empy state, is a neutral element for $\oplus$.
%We write $\varphi \# \varphi'$ if $\varphi \oplus \varphi'$ is defined,
%and $\varphi \succeq \varphi' \Longleftrightarrow (\exists \varphi'' \in \Sigma. \varphi = \varphi' \oplus \varphi'')$.
%We lift the operators $\oplus$ and $\succeq$ to sets of states $T$ and $U$, where
%$T \oplus U := \{ \varphi \oplus \varphi' | \varphi \in T \land \varphi' \in U \land \varphi \# \varphi' \}$ and
%$T \succeq U \Longleftrightarrow (\forall \varphi \in T. \exists \varphi' \in U. \varphi \succeq \varphi')$.
We define a partial order on elements of $\Sigma$ as follows:
A state $\sigma_2 \in \Sigma$ is \emph{greater than} a state $\sigma_1 \in \Sigma$, written $\sigma_2 \succeq \sigma_1$,
iff $\exists \sigma_r \in \Sigma \ldotp \sigma_2 = \sigma_1 \oplus \sigma_r$.
Moreover, we write $\sigma_1 \# \sigma_2$ iff $\sigma_1 \oplus \sigma_2$ is defined (i.e. $\sigma_1$ and $\sigma_2$ are compatible).
Finally, if $\sigma_2 \succeq \sigma_1$ then we define the subtraction $\sigma_2 \ominus \sigma_1$ to be the largest state $\sigma_r$ such that
$\sigma_2 = \sigma_1 \oplus \sigma_r$.

In order to enable a package algorithm to deconstruct the separating conjunctions and implications of the RHS of a wand,
and to extract the footprint piecewise as illustrated in \secref{subsec:fixing},
we consider an assertion language that contains the separating conjunction and the implication connectives.
This allows us to write logical rules that only apply to a separating conjunction and to an implication, respectively.
% The package logic contains a specific rule for each type of assertion.
Moreover, to be as general as possible, we do not fix the other connectives of the assertion language.
Thus, the third type of assertion we consider in our assertion language is the general type of semantic assertions, i.e. functions from $\Sigma$ to Booleans.
This third type represents any SL assertion that is neither a separating conjunction nor an implication.
In particular, assertions such as \code{x.f = 5}, \code{acc(x.f)}, abstract predicates (such as \code{Tree(x)}) or magic wands are represented as semantic assertions.
\thibault{Our assertion language is defined as
$A = A * A \mid \mathcal{B} \Rightarrow A \mid \mathcal{B}$,
where $A$ ranges over assertions and $\mathcal{B}$ over semantic assertions.
The semantics of this assertion language is defined in \appref{app:context}.}

This assertion language could be extended with the logical conjunction and the disjunction connectives,
to enable package algorithms to deconstruct these assertions as well.
We explain in \appref{app:extensions} how to extend the rules of the logic accordingly.
% Moreover, we explain in \appref{app:extensions} how to extend the rules of the logic and the syntax of assertions to handle the logical conjunction and disjunction.

%The point of defining (1) and (2) separately (since they can also be modelled with (3)) is to
%allow a package algorithm to deconstruct the assertions into smaller parts, in order to extract the footprint from the current state bit by bit.

%\subsection{Rules}\label{subsec:rules}
\subsection{The Logic}\label{subsec:logic}

The package logic generalises the approach described in \secref{subsec:fixing}, in order to capture many different strategies, as explained in \secref{subsec:motivation}.
\thibault{To package the wand $A \wand B$} in this generalised approach, a package algorithm starts in
\thibault{the initial context $(\sigma_0, S_0)$, where $\sigma_0$ (the outer state) corresponds to the current program state,
and $S_0$ (the initial witness set) contains the pair $(\sigma_A, e)$ for each $\sigma_A$ that satisfies $A$.}
Initially, the goal of a package algorithm is to extract from $\sigma_0$ a footprint $\sigma_w$ such that,
for all states $\sigma_A \in S_0^A$, if $\sigma_A \# \sigma_w$, then $\sigma_A \oplus \sigma_w \models B$.
To achieve this goal, the package algorithm traverses the assertion $B$ from left to right by deconstructing the separating conjunctions and implications inside $B$,
which leads to intermediate subgoals as shown in \secref{subsec:fixing}.
An intermediate subgoal for a package algorithm corresponds to a \emph{configuration}, which we formalise below.
% Intuitively, the configuration $\langle B, pc, (\sigma, S) \rangle


%We formalise this goal with a \emph{configuration}.

\paragraph{Configuration and reduction.}
A configuration is a triple $\langle B, pc, (\sigma, S) \rangle$, where $B$ is an assertion, $pc$ is a \emph{path condition} (i.e. a function from $\Sigma$ to Booleans), and $(\sigma, S)$ is a context.
The reason a configuration contains a path condition $pc$ is to enable a package algorithm to
\tout{deconstruct an implication into a smaller assertion,}
\thibault{do a case split on the LHS of an implication,} as we show below.
%Intuitively, the path condition $pc$ is the conjunction of all the conditions which guard the assertion $B$.
Thus, informally, a package algorithm in the configuration $\langle B, pc, (\sigma, S) \rangle$ must extract a state $\sigma_w$ from $\sigma$
such that all\footnote{\label{footnote:not_all_states} As we explain below, this condition does not apply to all states $\sigma_A$ for $(\sigma_A, \sigma_B) \in S_0$,
but only to those such that $(\sigma_A \oplus \sigma_B) \# \sigma_w$.}
states from $S^A$ combined with $\sigma_w$ satisfy the assertion $pc \Rightarrow B$.
The package logic describes the steps an algorithm is allowed to take to achieve this goal.
% presented in \figref{fig:package_rules},

The central feature of the package logic is the reduction of a configuration into a context,
written $\langle B, pc, (\sigma_0, S_0) \rangle \rightsquigarrow (\sigma_1, S_1)$, which describes the computation of a footprint of a wand.
$\langle B, pc, (\sigma_0, S_0) \rangle \rightsquigarrow (\sigma_1, S_1)$ informally means that the package algorithm has achieved its goal and found a footprint $\sigma_w$,
\thibault{which corresponds to the difference between $\sigma_0$ and $\sigma_1$.}
More precisely, the algorithm has found a state $\sigma_w$ (the footprint) such that $\sigma_0 = \sigma_1 \oplus \sigma_w$, and all\footnotemark[\ref{footnote:not_all_states}] states $\sigma_A \in S_0^A$ combined with $\sigma_w$
satisfy the assertion $pc \Rightarrow B$.
$S_1$ is the updated witness set, where $\sigma_w$ has first been combined with each element of $S_0^A$,
and the permissions \thibault{(with the corresponding values)} to satisfy $pc \Rightarrow B$ have then been transferred from the first element to the second element of each pair.


Therefore, to package the wand $A \wand B$ in the program state $\sigma_0$, the goal of an algorithm
is to find in the package logic a derivation of
\[
    \langle B, \lambda \sigma \ldotp \top, (\sigma_0, \{ (\sigma_A, e) \mid \sigma_A \models A \} ) \rangle \rightsquigarrow (\sigma_1, S_1)
\]
for some state $\sigma_1$ and witness set $S_1$.
The path condition is initially true, since we want to find a way to satisfy $B$.
Each pair of the initial witness set is composed of a state $\sigma_A$ that satisfies $A$, and the empty state $e$, to which a package algorithm will add permissions in order to satisfy $B$.
If $B$ is intuitionistic, the initial witness set might be simplified by only considering minimal states that satisfy $A$.
If the algorithm finds a proof of this reduction, it has proven that the difference between $\sigma_0$ and $\sigma_1$ is a valid footprint of the wand $A \wand B$,
since the logic is sound (\thmref{thm:soundness} below).

%\subsection{Rules}\label{subsec:rules}
\paragraph{Rules.}
\figref{fig:package_rules} presents the four rules of the package logic.
These rules describe how a configuration can be reduced to a context. There is a rule for each type of assertion.
The \emph{Implication} rule for an implication, the \emph{Star} rule for a separating conjunction, and the \emph{Atom} rule for a semantic assertion.
Finally, the rule \emph{Extract}, which can be applied with any assertion,
extracts resources from the outer state and combines these resources with all pairs of states from the witness set.
In the following, we informally write \emph{reducing an assertion}
to refer to the process of proving (in the logic) that the relevant configuration containing this assertion reduces to some context.
We explain in \appref{app:extensions} how the logic can be extended with two rules to deconstruct a disjunction and a logical conjunction, respectively, if the assertion language is extended accordingly.


\begin{figure}[t]
    \[
    \begin{array}{ll}

    \Inf[\mathit{Implication}]{\langle A,
    \lambda \sigma \ldotp pc(\sigma) \land b(\sigma), \Delta \rangle \rightsquigarrow \Delta'}
        {\langle b \Rightarrow A, pc, \Delta \rangle \rightsquigarrow \Delta'}


    %\\[3em]
    \hspace{10mm}

    \Inf[\mathit{Star}]{\langle A_1, pc, \Delta_0 \rangle \rightsquigarrow \Delta_1}.
        {\langle A_2, pc, \Delta_1 \rangle \rightsquigarrow \Delta_2}
        {\langle A_1 * A_2, pc, \Delta_0 \rangle \rightsquigarrow \Delta_2}


    \\[3em]

    \Inf[\mathit{Atom}]{\forall (\sigma_A, \sigma_B) \in S \ldotp pc(\sigma_A) \Longrightarrow \sigma_A \succeq \mathit{choice}(\sigma_A, \sigma_B) \land \mathcal{B}(\mathit{choice}(\sigma_A, \sigma_B))}.
        { S_{\top} = \{ (\sigma_A \ominus \mathit{choice}(\sigma_A, \sigma_B) , \sigma_B \oplus \mathit{choice}(\sigma_A, \sigma_B) ) | (\sigma_A, \sigma_B) \in S \land pc(\sigma_A) \} }.
        { S_{\bot} = \{ (\sigma_A, \sigma_B) | (\sigma_A, \sigma_B) \in S \land \lnot pc(\sigma_A) \} }
        {\langle \mathcal{B}, pc, (\sigma, S) \rangle \rightsquigarrow (\sigma, S_{\top} \cup S_{\bot})}



    \\[3em]

    \Inf[\mathit{Extract}]
    {\sigma_0 = \sigma_1 \oplus \sigma_w}{\textsf{stable}(\sigma_w)}{\langle A, pc, (\sigma_1, S_1) \rangle \rightsquigarrow \Delta}.
    {S_1 = \{ (\sigma_A \oplus \sigma_w, \sigma_B) | (\sigma_A, \sigma_B) \in S_0 \land (\sigma_A \oplus \sigma_B) \# \sigma_w \} }
        {\langle A, pc, (\sigma_0, S_0) \rangle \rightsquigarrow \Delta}


    \end{array}
    \]
    \caption{Rules of the Package Logic.}
    \label{fig:package_rules}
\end{figure}

The first two rules are quite straightforward.
For an implication $\mathcal{B} \Rightarrow A$, we conjoin the condition $\mathcal{B}$ with the path condition, and reduce the assertion $A$,
which informally expresses that satisfying the assertion $pc \Rightarrow (b \Rightarrow A)$ amounts to satisfying the assertion $(pc \land b) \Rightarrow A$ (\emph{Implication}).
For a separating conjunction $A_1 * A_2$, a package algorithm must reduce both $A_1$ and $A_2$, in order to reduce $A_1 * A_2$.
Therefore, the \emph{Star} rule constructs a state $\sigma_B$ that satisfies $A_1 * A_2$,
by first constructing a state $\sigma_1$ that satisfies $A_1$, and then combining it with a state $\sigma_2$ that satisfies $A_2$.
\thibault{The order in the premises of the \emph{Star} rule, i.e. handling $A_1$ before $A_2$, does not matter since $A_1 * A_2$ and $A_2 * A_1$ are equivalent.
The logic could thus be soundly extended with a rule that proceeds $A_2$ before $A_1$.}

Informally, the \emph{Atom} rule specifies how to prove that all states in $S^A$ (where $S$ is the witness set) satisfy the assertion $pc \Rightarrow \mathcal{B}$.
\tout{We first separate the witness set $S$ into two witness sets,
depending on whether the first element of a pair satisfies the path condition $pc$.
If it does not, then it does not have to satisfy the semantic assertion $\mathcal{B}$ either,
thus these pairs of states (which belong to the witness set $S_{\bot}$) are left unchanged.
For each pair of states $(\sigma_A, \sigma_B) \in S$ whose first element satisfies the path condition (i.e. $pc(\sigma_A)$ holds),
we must \emph{choose} a state smaller or equal to $\sigma_A$ to satisfy $\mathcal{B}$:
This choice is expressed with $\mathit{choice}(\sigma_A, \sigma_B)$, where the function $choice$ is a parameter of the rule.
Choosing the function $choice$ amounts to choosing how to satisfy the assertion $\mathcal{B}$ for each relevant pair of states.
In the end, we transfer $\mathit{choice}(\sigma_A, \sigma_B)$ from $\sigma_A$ to $\sigma_B$, as expressed in the definition of $S_{\top}$.}
\thibault{More precisely, consider a pair $(\sigma_A, \sigma_B) \in S$.
If $\sigma_A$ does not satisfy the path condition, i.e. $\lnot pc(\sigma_A)$, then $\sigma_A$ \emph{does not} have to justify $\mathcal{B}$,
and thus the pair $(\sigma_A, \sigma_B)$ is left unchanged.
This case corresponds to the set $S_\bot$.
On the other hand, if $\sigma_A$ satisfies the path condition, i.e. $pc(\sigma_A)$, then $\sigma_A$ must satisfy $\mathcal{B}$,
and the corresponding permissions must be transferred from $\sigma_A$ to $\sigma_B$.
Since some SL assertions may be satisfied in different ways, such as disjunctions, the algorithm has a choice in how
to satisfy $\mathcal{B}$, which might be different for each pair $(\sigma_A, \sigma_B)$.
Thus, this choice is expressed with $\mathit{choice}(\sigma_A, \sigma_B)$.
$\mathit{choice}(\sigma_A, \sigma_B)$ must be smaller or equal to $\sigma_A$, and it must satisfy $\mathcal{B}$.
We update the witness set by transferring $\mathit{choice}(\sigma_A, \sigma_B)$ from $\sigma_A$ to $\sigma_B$.
This second case corresponds to the set $S_\top$.
Note that the \emph{Atom} rule can only be applied if $\sigma_A$ satisfies $\mathcal{B}$, for all pairs $(\sigma_A, \sigma_B) \in S$ such that $pc(\sigma_A)$.
It this rule cannot be applied, a package algorithm must either extract more permissions from the outer state with the \emph{Extract} rule, or fail.}


Finally, the $\mathit{Extract}$ rule states that, at any step of the derivation, we can extract resources
(represented by the \emph{stable} state $\sigma_w$) from the outer state $\sigma_0$, and combine these resources with all pairs of states in the witness set.
\thibault{We explain formally in \appref{app:context} what is a stable state and why the extracted state $\sigma_w$ must be stable.
Informally, it simply means that $\sigma_w$ only contains the values of heap locations to which it has some permission.}
%The algorithm can then add the transformed partial footprint, $t(\sigma_w') \ominus t(\sigma_w)$,
Note that, if $\sigma_A \oplus \sigma_B$ cannot be combined with $\sigma_w$, then we remove this pair of states from the witness set.
\tout{The fact that this addition is inconsistent means that the assumptions underlying this state are inconsistent, and thus any assertion can be proven from these.}
\thibault{The reason is that $\sigma_A \oplus \sigma_B$ corresponds, at any point of the derivation,
to the combination of a state $\sigma_A'$ that satisfies $A$ with the footprint $\sigma_f$ extracted so far.
Therefore, if $\sigma_A \oplus \sigma_B$ cannot be combined with $\sigma_w$,
it means that the initial state $\sigma_A'$ is not compatible with the new footprint extracted so far, $\sigma_f \oplus \sigma_w$.
Thus, $\sigma_A' \oplus \sigma_f \oplus \sigma_w = \sigma_A \oplus \sigma_B \oplus \sigma_w$ does not have to satisfy the RHS of the wand,
by definition of the magic wand.}
This is the reason why a witness set tracks the pairs of states $(\sigma_A, \sigma_B)$, instead of simply tracking $\sigma_A$.
Finally, we reduce the assertion $A$ in the new context.

\thibault{The strategy of a package algorithm is mostly reflected in when and how a package algorithm uses the \emph{Extract} rule.
As an example, to package the wand $\code{acc(x.b, 1/2)} \wand \code{acc(x.b, 1/2)} * (\code{x.b} \Rightarrow \code{acc(x.f)})$ from \secref{subsec:motivation},
one algorithm might use this rule to extract permission to \code{x.f}, while another algorithm might use it to extract
permission to \code{x.b} (if \code{x.b} contains the value false in the outer state).
We show in \appref{app:example-derivation}, as an example, a part of the derivation in the package logic that corresponds to the example from \secref{subsec:fixing}.}





\subsection{Soundness and Completeness}\label{subsec:soundness-completeness}

As explained above, the goal of a package algorithm is to find a proof of
$\langle B, \lambda \_ \ldotp \top, (\sigma, \{ (\sigma_A, e) \mid \sigma_A \in S_A \}) \rangle \rightsquigarrow (\sigma', S')$.
The package logic is sound.
Simply put, this means that if there exists in the logic a derivation of this reduction,
then there exists a state $\sigma_w$ (the footprint) such that $\sigma = \sigma' \oplus \sigma_w$
and, for all states $\sigma_A \in S_A$, if $\sigma_A$ and $\sigma_w$ are compatible,
then $\sigma_A \oplus \sigma_w$ satisfies $B$.
In particular, if $S_A$ contains all states that satisfy $A$, then the difference between $\sigma$ and $\sigma'$ is a stable footprint of $A \wand B$.

We write $\vdash \langle B, pc, \Delta \rangle \rightsquigarrow \Delta'$ to state that a reduction can be proven in the logic.
We have proven the following soundness result in Isabelle/HOL:
%\footnote{Recall \label{note:simplified}
%that we present in this section a simplified version of the mechanised theory.
%This simplification focuses on the usual definition of the wand.
%\secref{sec:combinable} explains how to extend the theory to handle other definitions.}

\begin{theorem}\textbf{Soundness}. \label{thm:soundness}
    Let $S_A$ be a set of states. If
    \begin{enumerate}
        \item the assertion $B$ is well-formed\protect\footnote{\label{note:wf}We formally define well-formedness in \appref{app:context}.
        \thibault{Intuitively, a well-formed assertion roughly corresponds to a self-framing assertion as defined in \secref{subsec:idf_background}.}
        \tout{an assertion is well-formed if, in a state in which it is well-defined, adding information about heap values to this state does not change
        whether the assertion holds or not.}},
        \item $\vdash \langle B, \lambda \_ \ldotp \top, (\sigma, \{ (\sigma_A, e) \mid \sigma_A \in S_A \}) \rangle \rightsquigarrow (\sigma', S')$, and
        \item one of the following condition holds:
            \begin{enumerate}
                \item $B$ is intuitionistic
                \item For all $(\sigma_A, \sigma_B) \in S'$, $\sigma_A$ contains no permission (i.e. $\sigma_A \oplus \sigma_A = \sigma_A$)
            \end{enumerate}
    \end{enumerate}
    then there exists $\sigma_w \in \Sigma$ such that
    \thibault{(1) $\textsf{stable}(\sigma_w)$,
    (2) $\sigma = \sigma' \oplus \sigma_w$, and
    (3) $\forall \sigma_A \in S_A \ldotp \sigma_A \# \sigma_w \Longrightarrow \sigma_A \oplus \sigma_w \models B$.}
    \tout{
    \begin{enumerate}
        \item $\textsf{stable}(\sigma_w)$,
        \item $\sigma = \sigma' \oplus \sigma_w$, and
        \item $\forall \sigma_A \in S_A \ldotp \sigma_A \# \sigma_w \Longrightarrow \sigma_A \oplus \sigma_w \models B$.
    \end{enumerate}
    }
\end{theorem}

A proof sketch of this result is given in \appref{app:proofs}.
The third premise shows that, in an intuitionistic SL or in IDF,
the correspondence between a proof in the logic and a valid footprint of a wand is straighforward:
If $S_A$ contains all states that satisfy the assertion $A$, i.e.
$\forall \sigma_A \in \Sigma \ldotp \sigma_A \models A \Longrightarrow \sigma_A \in S_A$, then $\sigma_w$ is a footprint of the wand $A \wand B$.
In classical SL, as shown by the disjunction, one must in general additionally check that all resources in the witness set have been ``consumed''.

\begin{comment}
\begin{corollary}
    If
    \begin{enumerate}
        \item the assertion $B$ is well-formed\footnotemark[\ref{note:wf}],
        \item $\forall \sigma_A \in \Sigma \ldotp \sigma_A \models A \Longrightarrow \sigma_A \in S_A$,
        \item $\vdash \langle B, \lambda \_ \ldotp \top, (\sigma, \{ (\sigma_A, e) \mid \sigma_A \in S_A \}) \rangle \rightsquigarrow (\sigma', S')$, and
        \item one of the following condition holds:
            \begin{enumerate}
                \item $B$ is intuitionistic
                \item For all $(\sigma_A, \sigma_B) \in S'$, $\sigma_A$ has no ownership (i.e. $\sigma_A \oplus \sigma_A = \sigma_A$)
            \end{enumerate}
    \end{enumerate}
    then there exists $\sigma_w \in \Sigma$ such that $\sigma = \sigma' \oplus \sigma_w$ and
    $\sigma_w$ is a stable footprint of the wand $A \wand B$.
\end{corollary}
\end{comment}

%\subsection{Completeness}\label{subsec:completeness}

We have proven in Isabelle/HOL that the package logic is also complete:
%\footnotemark[\ref{note:simplified}]:
%it means that if there exists $\sigma_w \in \Sigma$
%such that $\textsf{stable}(\sigma_w)$ and $\forall \sigma_A \in S_A \ldotp \sigma_A \# \sigma_w \Longrightarrow \sigma_A \oplus \sigma_w \models B$,
%then there exists a proof of
%$\langle B, \lambda \_ \ldotp \top, (\sigma, \{ (\sigma_A, e) \mid \sigma_A \in S_A \}) \rangle \rightsquigarrow (\sigma', S')$:

\begin{comment}
\begin{theorem}\textbf{Completeness}.\\
    \label{thm:completeness}
    Let $S \subseteq \Sigma$ be a set of states and $\sigma_w \in \Sigma$ a state.
    If
    \begin{enumerate}
        \item $\forall \sigma_A \in S \ldotp \sigma_A \# \sigma_w \Longrightarrow \sigma_A \oplus \sigma_w \models B$,
        \item $\sigma = \sigma' \oplus \sigma_w$,
        \item $\sigma_w$ is stable, i.e. $\textsf{stable}(\sigma_w)$, and
        \item the assertion $B$ is well-formed\footnotemark[\ref{note:wf}],
    \end{enumerate}
    then there exists a witness set $S'$ such that the following holds:
\[
    \vdash \langle B, \lambda \_ \ldotp \top, (\sigma, \{ (\sigma_A, e) \mid \sigma_A \in S_A \}) \rangle \rightsquigarrow (\sigma', S')
\]
\end{theorem}
\end{comment}

%This result implies, in particular, that any stable and valid footprint can be computed using the rules of the logic:

% \begin{corollary}
\begin{theorem}\textbf{Completeness}.
    \label{thm:completeness}
    If
    \begin{enumerate}
        \item $\sigma_w$ is a stable footprint of $A \wand B$,
        \item $\sigma = \sigma' \oplus \sigma_w$, and
        \item the assertion $B$ is well-formed\footnotemark[\ref{note:wf}],
    \end{enumerate}
    then there exists a witness set $S'$ such that the following holds:
    \[
        \vdash \langle B, \lambda \_ \ldotp \top, (\sigma, \{ (\sigma_A, e) \mid \sigma_A \in S_A \}) \rangle \rightsquigarrow (\sigma', S')
    \]
\end{theorem}

A proof sketch of this result is given in \appref{app:proofs}. 


